GNNExplainer: Generating Explanations for Graph Neural Networks

Graph Neural Networks (GNNs) are a powerful tool for machine learning on graphs.GNNs combine node feature information with the graph structure by recursively passing neural messages along edges of the input graph. However, incorporating both graph structure and feature information leads to complex models, and explaining predictions made by GNNs remains unsolved. Here we propose GNNExplainer, the first general, model-agnostic approach for providing interpretable explanations for predictions of any GNN-based model on any graph-based machine learning task. Given an instance, GNNExplainer identifies a compact subgraph structure and a small subset of node features that have a crucial role in GNN's prediction. Further, GNNExplainer can generate consistent and concise explanations for an entire class of instances. We formulate GNNExplainer as an optimization task that maximizes the mutual information between a GNN's prediction and distribution of possible subgraph structures. Experiments on synthetic and real-world graphs show that our approach can identify important graph structures as well as node features, and outperforms baselines by 17.1% on average. GNNExplainer provides a variety of benefits, from the ability to visualize semantically relevant structures to interpretability, to giving insights into errors of faulty GNNs.

==> 030background.tex <==
\section{Background}
\label{sec:background}

% We first give an overview of the formulation of \gnn models. 

% Maybe merge with Background
\xhdr{Graph Neural Networks} Graph Neural Networks (\gnn)~\cite{scarselli} obtain node embeddings by recursively propagating information from its neighbours. This framework was later unified into a general Neural Message-Passing scheme~\cite{gilmer2017neural}, and more recently into the relational inductive bias model~\cite{battaglia}. For a more detailed review of recent developments we please refer the reader to~\cite{zhang_deep_2018, zhou_graph_2018, battaglia,hamilton2017representation}.
%
Under this model, \gnns have achieved state-of-the-art performance across a variety of tasks, such as node classification~\cite{kipf2016semi, graphsage}, link prediction~\cite{zhang2018link, schlichtkrull2018modeling}, graph clustering~\cite{defferrard2016convolutional, ying2018hierarchical} or graph classification~\cite{ying2018hierarchical, dai2016discriminative, duvenaud_convolutional_2015}. These tasks occur in domains where the graph structure is ubiquitous, such as social networks~\cite{backstrom2011supervised}, content graphs~\cite{pinsage}, biology~\cite{agrawal2018large}, and chemoinformatics~\cite{duvenaud_convolutional_2015,jin2017predicting,zitnik2018decagon}.
%
Recent instances of \gnn models have been proposed to augment the interpretability properties of \gnns~\cite{PhysRevLett.120.145301, neil2018interpretable, velickovic2018graph}. However, in contrast to our work here, \rex{these approaches are limited to their own \gnn architecture, and cannot make explanations using both features and subgraph structure jointly.}
%these approaches design a novel \gnn architectures explicitly for the purpose of interpretability. 
\rex{Notably, although the edge attention values in graph attention networks can serve as indication of structure importance, it is the same for predictions on all nodes. Thus it contradicts with many application scenario where an edge is important for predictions on one node, but not the other.
(or maybe move to experiments)}
\rex{remove?} Our goal here is different, as we are already given a trained model in the \gnn-family and aim to explain its predictions.
%, an approach that is at odds with our goal of post-hoc interpretation for any generic \gnn~ model.

\xhdr{General Formulation of GNNs}
%
A per-layer update of a \gnn model involves three key computations~\cite{battaglia,zhang_deep_2018,zhou_graph_2018}:
%
\begin{align}
    m_{ij}^l & = \textsc{Msg}(\mathbf{h}_i^{l-1}, \mathbf{h}_j^{l-1}, r_{ij}) \label{eq:msg} \\   
    M_{i}^l & = \textsc{Agg}(\{m_{ij}^l | v_j \in \mathcal{N}_{v_i}\}) \label{eq:agg} \\
    \mathbf{h}_{i}^l & = \textsc{Update}(M_i^l, \mathbf{h}_i^{l-1}) \label{eq:update}
\end{align}
%
First, the model computes neural messages between every pair of nodes (Equation~\ref{eq:msg}). The message for node pair $(v_i, v_j)$ is a function of $v_i$'s  and $v_j$'s representations $\mathbf{h}_i^{l-1}$ and $\mathbf{h}_j^{l-1}$ in the previous layer, and the relation $r_{ij}$ between the nodes. In different \gnn models, $r_{ij}$ can indicate, for example, an edge type~\cite{zitnik2018decagon}, an edge weight~\cite{pinsage}, or a shortest path from $v_i$ to $v_j$. Second, for each node $v_i$, the \gnn model aggregates messages from $v_i$'s neighborhood $\mathcal{N}_{v_i}$ and calculates an aggregated message $M_i$ (Equation~\ref{eq:agg}). Popular aggregation methods include mean/max pooling~\cite{graphsage}, permutation invariant neural networks, and Recurrent Neural Networks~\cite{xu2018powerful}. 

Here, the definition of a node neighborhood $\mathcal{N}$ is crucial, as it can affect the performance and scalability of the \gnn model. Popular definitions include immediate network neighborhoods~\cite{kipf2016semi}, multi-hop neighborhoods~\cite{xujumping}, sampling-based neighborhoods~\cite{fastgcn, Chen2018StochasticTO, Huang2018AdaptiveST, graphsage}, or PageRank-based neighborhoods~\cite{pinsage}. Finally, the \gnn model takes the aggregated message $M_i^l$ along with $v_i$'s representation $\mathbf{h}_i^{l-1}$ from the previous layer, and it non-linearly transforms them to obtain $v_i$'s representation $\mathbf{h}_i^l$ at layer $l$ (Equation~\ref{eq:update}).

These computations are performed for every layer, with the initial condition $\mathbf{h}_i^0 = \mathbf{x}_i$, where $\mathbf{x}_i$ is initial node feature vector. The final embedding for node $v_i$ after $L$ layers of computation is $\mathbf{z}_i = \mathbf{h}_i^L$. To predict the label for node $i$, we pass the node embedding $\mathbf{z}_i$ through a standard classification network, such as a multi-layer perceptron (MLP) with a softmax output layer. Our \name is a model-agnostic framework that provides explanations for any \gnn that can be formulated in terms of Equations~\ref{eq:msg}--\ref{eq:update}.

\xhdr{Computation Graphs}
%
In the context of a neural network architecture, the information that a \gnn~ relies on for computing $\mathbf{z}_i$ is completely determined by $v_i$'s computation graph, which is defined by Equation~\ref{eq:agg}. The \gnn uses that computation graph to generate $v_i$'s representation $\mathbf{z}_i$ (Equations~\ref{eq:msg} and~\ref{eq:update})~\cite{zhang_deep_2018, zhou_graph_2018}. Importantly, the structure of the computation graph is different for each node $v_i$, and depends on how the neighborhood $\mathcal{N}_{v_i}$ is defined. Let $G_c(v_i)$ denote the computation graph used by the \gnn~ to compute representation $\mathbf{z}_i$ of node $v_i$.
The $G_c(v_i)$ can be obtained by performing a graph traversal of arbitrary depth $L$, \eg, a Breadth-First Search (BFS), using $\mathcal{N}_{v_i}$ as the neighborhood definition. We further define $A_c(v_i)$ as the adjacency matrix corresponding to the computation graph $G_c(v_i)$.

Following this definition, in Graph Convolutional Networks (GCNs)~\cite{kipf2016semi}, the computation graph $G_c(v_i)$ is simply an $L$-hop neighborhood of $v_i$ in the input graph $G$. However, in other \gnn models, such as Jumping Knowledge Networks~\cite{xujumping}, attention-based networks~\cite{velickovic2018graph}, and Line-Graph NNs~\cite{chen2018supervised}, the computation graph $G_c(v_i)$ will be different from the exhaustive $L$-hop neighborhood.

\hide{
We first give a brief overview of the general formulation of \gnn~ architectures. 

\subsection{Graph Neural Networks (GNNs)}

As summarized in reviews \cite{battaglia,zhang_deep_2018,zhou_graph_2018}, \gnn~ models are generally composed of three components. 
At each layer, the model computes messages (Equation \ref{eq:msg}) between a pair of nodes $(v_i, v_j)$, which is a function of $\mathbf{h}_i^{l-1}$, $\mathbf{h}_j^{l-1}$, the representations of $v_i$ and $v_j$ at the previous layer, and the relation $r_{ij}$ between $v_i$ and $v_j$.
In different variations of \gnn s, $r_{ij}$ could indicate for example the edge type\cite{zitnik2018decagon}, edge weights\cite{pinsage}, or a shortest path from $v_i$ to $v_j$~\CITE.

For each node $v_i$, the \gnn~ aggregates the messages incoming from nodes in its neighborhood $\mathcal{N}_{v_i}$ by Equation~\ref{eq:agg}. Common aggregation methods include mean/max pooling~\cite{graphsage}, permutation invariant or equivariant neural networks such as DeepSets~\cite{deepsets} and Set2Set~\cite{vinyals2015order}, Recurrent Neural Networks (RNNs). The choice of a neighborhood is also crucial, notably for performance. Many designs choices have been explored, including using the immediate neighborhood, a multi-hop neighborhood\CITE, sampling-based neighborhoods~\cite{fastgcn, Chen2018StochasticTO, Huang2018AdaptiveST}, or PageRank-based neighborhoods~\cite{pinsage}.

Finally, an update function (Equation~\ref{eq:update}) takes the aggregated message $M_i$ and the representation of $v_i$ at the previous layer as input, and performs a non-linear transformation to obtain $v_i$'s representation $\mathbf{h}_i^l$ at layer $l$.
%
\begin{equation}
    \label{eq:msg}
    m_{ij}^l = \textsc{Msg}(\mathbf{h}_i^{l-1}, \mathbf{h}_j^{l-1}, r_{ij})
\end{equation}
\begin{equation}
    \label{eq:agg}
    M_{i}^l = \textsc{Agg}(\{m_{ij}^l | v_j \in \mathcal{N}_{v_i}\})
\end{equation}
\begin{equation}
    \label{eq:update}
    \mathbf{h}_{i}^l = \textsc{Update}(M_i^l, \mathbf{h}_i^{l-1})
\end{equation}
%
These three computation steps are performed for every layer, with the initial condition $\mathbf{h}_i^0 = \mathbf{x}_i$.
The final embedding $\mathbf{z}_i = \mathbf{h}_i^L$ is then passed through a standard classification network, such as multi-layer perceptron (MLP) with a softmax output layer, yielding the predicted label for node $v_i$.
\name represents a general framework that is able to provide explanations for any existing \gnn s built around the aforementioned components.

\subsection{Neural Computation Graphs}

In terms of neural network architecture, we can view Equation~\ref{eq:agg} as defining a computation graph for evaluating a representation of node $v_i$ \CITE, while Equations~\ref{eq:msg} and~\ref{eq:update} define operators on this computation graph. \rex{figure explanation}

The structure of the computation graph is different for each node $v_i$, and depends on how the neighborhood $\mathcal{N}(v_i)$ is defined. Let $G_c(v_i)$ denote the computation graph used by the \gnn~ to compute representation $\mathbf{h}_i$ of node $v_i$.
$G_c(v_i)$ can be obtained by performing a graph traversal of arbitrary depth $L$, e.g. a Breadth-First Search (BFS), using $\mathcal{N}$ as the neighborhood definition.
We further define $Ac(v_i)$ as the adjacency matrix corresponding to the computation graph $G_c(v_i)$.

Following this definition, in a Graph Convolutional Network (GCN)~\cite{kipf2016semi}, the computation graph is simply the $L$-hop neighborhood of $v_i$ in the input graph $G$. However, in other variants such as Jumping Knowledge Networks~\cite{xujumping}, attention-based networks~\cite{velickovic2018graph}, or Line-Graph Neural Networks~\cite{chen2018supervised}, the computation graph will be very different from the exhaustive $L$-hop neighborhood.

The information that a \gnn~ relies on for computing $\mathbf{h}_i^L$ can be completely described by its computation graph $G_c(v_i)$ and the associated feature set $X_c(v_i) = \{x_j | v_j \in G_c(v_i)\}$.\dylan{should we specify the case of the node's self features?}

We thus use these elements as inputs to the \gnn~model $\hat{y} = \Phi(G_c(v_i), X_c(v_i))$.
Therefore, when constructing local explanation for \gnn~ prediction made on $v_i$, we only consider structural information present in $G_c(v_i)$, and node features from $X_c(v_i)$.
}
